Networked Computing in Wireless Sensor Networks for Structural Health Monitoring

This paper studies the problem of distributed computation over a network of wireless sensors. While this problem applies to many emerging applications, to keep our discussion concrete we will focus on sensor networks used for structural health monitoring. Within this context, the heaviest computation is to determine the singular value decomposition (SVD) to extract mode shapes (eigenvectors) of a structure. Compared to collecting raw vibration data and performing SVD at a central location, computing SVD within the network can result in significantly lower energy consumption and delay. Using recent results on decomposing SVD, a well-known centralized operation, into components, we seek to determine a near-optimal communication structure that enables the distribution of this computation and the reassembly of the final results, with the objective of minimizing energy consumption subject to a computational delay constraint. We show that this reduces to a generalized clustering problem; a cluster forms a unit on which a component of the overall computation is performed. We establish that this problem is NP-hard. By relaxing the delay constraint, we derive a lower bound to this problem. We then propose an integer linear program (ILP) to solve the constrained problem exactly as well as an approximate algorithm with a proven approximation ratio. We further present a distributed version of the approximate algorithm. We present both simulation and experimentation results to demonstrate the effectiveness of these algorithms.

==> abstract.tex <==
TO BE ADDED 


==> related.tex <==
\section{Related Work}
\label{sec:related}

Prior works which study deriving the communication structure with in-network computation belong to one of the following
three catefories. (i) They consider only very simple functions like max/min/average/median (for example, see~\cite{tag,median:podc,max:pods,wang:convergcast} and
references therein) that do not represent the complex computational requirements demanded by practical 
engineering applications like structural health monitoring. (ii) They study scaling laws which do not yield algorithms to determine the optimal communication
structure~\cite{kumar:scaling}. (iii) They study algorithms to derive the communication structure with data compression/compressed 
sensing~\cite{bazarul:ton,sivakumar:secon,pattem:ipsn}. These algorithms are directly relevant to the study of peak-picking, but 
cannot be used to derive the communication structure for the SVD computation as they do not have any constraint equivalent to the combinability
constraint in the SVD computation. Moreover, they do not incorporate any computational delay constraint. 
Thus, the presence of more complex constraints like combinability as well as the requirement of optimizing energy under a \emph{computational delay constraint}
makes this work very different from prior works. 
%which study the communication structure with in-network computation. 

\noindent {\bf Degree-Constrained Data Collection Tree: } We study this problem in the context of deriving an 
approximate communication structure with in-network computation. However, note that this is an important
problem in its own right and has other applications in wireless sensor systems, like building a data collection
tree to minimize interference when multiple frequency channels are available for scheduling~\cite{bhaskar:freq}. 
Results for this problem are known only for complete graphs whose weights satisfy the triangle inequality~\cite{tree:apx,helmick:multicast}.
Hence, our work is the first to propose approximation algorithms and analytically derive their approximation
factors for this problem in graphs induced by a communication network.  
 

